Verifiable Differential Privacy

Differential Privacy (DP) is often presented as a strong privacy-enhancing technology with broad applicability and advocated as a de-facto standard for releasing aggregate statistics on sensitive data. However, in many embodiments, DP introduces a new attack surface: a malicious entity entrusted with releasing statistics could manipulate the results and use the randomness of DP as a convenient smokescreen to mask its nefariousness. Since revealing the random noise would obviate the purpose of introducing it, the miscreant may have a perfect alibi. To close this loophole, we introduce the idea of \textit{Verifiable Differential Privacy}, which requires the publishing entity to output a zero-knowledge proof that convinces an efficient verifier that the output is both DP and reliable. Such a definition might seem unachievable, as a verifier must validate that DP randomness was generated faithfully without learning anything about the randomness itself. We resolve this paradox by carefully mixing private and public randomness to compute verifiable DP counting queries with theoretical guarantees and show that it is also practical for real-world deployment. We also demonstrate that computational assumptions are necessary by showing a separation between information-theoretic DP and computational DP under our definition of verifiability.

==> tex_files/mpc_dp_definitions.tex <==
\section{Verifiable Differential Privacy with Client-Server MPC}

A well-known disadvantage of DP in the trusted curator model is that a single entity has full access to the data. Thus, a client cannot verify if the data used to publish statistics has been computed using the same data that the clients originally submitted. Furthermore, as the single server sees all the data in plaintext, they might disclose this information to an adversary for a profit later \cite{dataSold}. Thus instead, DP using MPC allows $n$ clients to secret share their inputs between $K \geq 2$ servers using any linear secret sharing scheme. As long as a single server is honest, the servers learn no Shannon information about an honest client's input. The query $Q$ is now securely computed using an MPC protocol $\Pi_Q$ such the servers learn nothing but a DP version of $Q(X_1, \dots, X_k)$ where $X= \sum_{i=1}^K X_i$. The marriage between MPC and DP is not new. In fact it was proposed by \cite{dwork2006our} and has seen widspread adoption for real-world tasks \cite{boneh_lightweight_2022, corrigan-gibbs_prio_2017, davidson2021star, bell2022distributed, roy2020crypt, bohler2020secure, boneh2019zero}. Despite the large body of work in MPC-DP, verifying whether the output is both DP and has the prescribed error remains unexplored. Thus, we extend the idea of verifiable differential DP from a single curator model to an MPC model as follows:





==> tex_files/schnorr.tex <==
\pdfoutput=1

\parag{Schnorr Sigma Protocols}

\parag{Unifying proofs of knowledge/Fiat Shamir}

\parag{Pedersen Commitments}
\label{sec: commitments}
Let $g$ be a generator of $\G_q$ and $h$ be a random element of $\G_q$. For $r \xleftarrow[]{R} \Z_q$, a Pedersen commitment to $s \in \Z_q$ is defined as 
\begin{equation}
    \Com(s, r) = g^sh^r = c
\end{equation}
    
The commitment has the following properties:
\begin{theorem}
\cite{pedersen1991non} For any $s \in \Z_q$ and $r \xleftarrow[]{R} \Z_q$, $\Com(s, r)$ is uniformly distributed in $\G_q$. Therefore the commitment is information-theoretically hiding. 
\end{theorem}

\begin{theorem}
\label{theorem: computational_binding}
\cite{pedersen1991non}
Any adversary $\mathcal{A}$ that can break Pedersen commitments can also win the \text{DLog} game with non-negligible probability. More formally, given $\Com(s,r)$ if $\mathcal{A}$ can find $(s^\prime, r^\prime)$ such that $\Com(s,r) = \Com(s^\prime,r^\prime)$ with probability $\rho$, then $\mathcal{A}$ is able to win the \text{DLog} game with probability $\rho$. Thus the commitment is computationally bounding.
\end{theorem}

\textbf{Notation}: For a vector $\bvec{s} \in \Z_q^M$ and i.i.d random values $\bvec{r} \xleftarrow[]{R} \Z_q^M$, when we write $\Com(\bvec{s}, \bvec{r}) \in G_q^M$ we mean coordinatewise commitments of $\bvec{s}$ using $\bvec{r}$ i.e., for each $j \in [M]$, $\Com(s_j, r_j) = g^{s_j}g^{r_j}$.


